Semantic Segmentation with Active Semi-Supervised Learning

Using deep learning, we now have the ability to create exceptionally good semantic segmentation systems; however, collecting the prerequisite pixel-wise annotations for training images remains expensive and time-consuming. Therefore, it would be ideal to minimize the number of human annotations needed when creating a new dataset. Here, we address this problem by proposing a novel algorithm that combines active learning and semi-supervised learning. Active learning is an approach for identifying the best unlabeled samples to annotate. While there has been work on active learning for segmentation, most methods require annotating all pixel objects in each image, rather than only the most informative regions. We argue that this is inefficient. Instead, our active learning approach aims to minimize the number of annotations per-image. Our method is enriched with semi-supervised learning, where we use pseudo labels generated with a teacher-student framework to identify image regions that help disambiguate confused classes. We also integrate mechanisms that enable better performance on imbalanced label distributions, which have not been studied previously for active learning in semantic segmentation. In experiments on the CamVid and CityScapes datasets, our method obtains over 95% of the network's performance on the full-training set using less than 17% of the training data, whereas the previous state of the art required 40% of the training data.

==> WACV 2023/fig/cityscapes_selections.tex <==
\begin{figure}[t]
    \centering
    \begin{subfigure}[t]{0.23\linewidth}
        \begin{center}
        \includegraphics[width=\linewidth]{pathtofigs/cityscapes_selections/69.png}
        \end{center}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.23\linewidth}
        \begin{center}
        \includegraphics[width=\linewidth]{pathtofigs/cityscapes_selections/112.png}
        \end{center}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.23\linewidth}
        \begin{center}
        \includegraphics[width=\linewidth]{pathtofigs/cityscapes_selections/1862.png}
        \end{center}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.23\linewidth}
        \begin{center}
        \includegraphics[width=\linewidth]{pathtofigs/cityscapes_selections/2072.png}
        \end{center}
    \end{subfigure}
    \par\medskip
    \begin{subfigure}[t]{0.23\linewidth}
        \begin{center}
        \includegraphics[width=\linewidth]{pathtofigs/cityscapes_selections/69_mask.png}
        \end{center}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.23\linewidth}
        \begin{center}
        \includegraphics[width=\linewidth]{pathtofigs/cityscapes_selections/112_mask.png}
        \end{center}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.23\linewidth}
        \begin{center}
        \includegraphics[width=\linewidth]{pathtofigs/cityscapes_selections/1862_mask.png}
        \end{center}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.23\linewidth}
        \begin{center}
        \includegraphics[width=\linewidth]{pathtofigs/cityscapes_selections/2072_mask.png}
        \end{center}
    \end{subfigure}
    \par\medskip
    \begin{subfigure}[t]{0.23\linewidth}
        \begin{center}
        \includegraphics[width=\linewidth]{pathtofigs/cityscapes_selections/69_drn.png}
        \end{center}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.23\linewidth}
        \begin{center}
        \includegraphics[width=\linewidth]{pathtofigs/cityscapes_selections/112_drn.png}
        \end{center}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.23\linewidth}
        \begin{center}
        \includegraphics[width=\linewidth]{pathtofigs/cityscapes_selections/1862_drn.png}
        \end{center}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.23\linewidth}
        \begin{center}
        \includegraphics[width=\linewidth]{pathtofigs/cityscapes_selections/2072_drn.png}
        \end{center}
    \end{subfigure}
\caption{\textbf{Regions:} Set of images showing what areas were chosen to be sampled in CityScapes over 5 active learning cycles with MobileNetv2 (2nd row) and DRN (3rd row). Our approach focuses on regions with high value information, still having uniqueness with areas acquisitioned depending on the backbone being used.}
\label{fig:selection_cityscapes_regions}
\end{figure}

==> WACV 2023/fig/overview-detail.tex <==
\begin{figure*}[t]
\begin{center}
\includegraphics[width=0.95\linewidth]{pathtofigs/fig_main.pdf}
\end{center}
\caption{
% 
Our SSL setup with (a) teacher-student framework, where (b) shows Confidence Weighting on a per-pixel basis, where the overall cross-entropy loss is weighted by the highest probability for the corresponding pseudo label (blue indicates high, and green indicates low), and (c) shows the Balanced ClassMix, where we maintain a replay buffer of unlabeled images and randomly sample them for ClassMix to further boost the number of samples for tail classes.}
\label{fig:algooverviewdetail}
\end{figure*}

==> WACV 2023/fig/results_main.tex <==
\begin{figure*}
    \begin{subfigure}[t]{0.48\textwidth}
    \begin{center}
    \includegraphics[width=\linewidth]{pathtofigs/performance_camvid.pdf}
    \end{center}
    \caption{CamVid}
    \label{fig:results_camvid_main}
    \end{subfigure}
    \begin{subfigure}[t]{0.48\textwidth}
    \begin{center}
    \includegraphics[width=\linewidth]{pathtofigs/performance_cityscapes.pdf}
    \end{center}
    \caption{CityScapes}
    \label{fig:results_cityscapes_main}
    \end{subfigure}
    \caption{\textbf{IoU:} Performance curves of using pseudo labels as a function of the total data used for training on (a) CamVid and (b) CityScapes. We reduce the labeling effort significantly, by requiring only $\sim$4\% and 6\% additional data on both datasets respectively. On the same initial data, the best state-of-the-art method achieves comparative performance with an additional 30\% data.}
\end{figure*}

% \begin{figure}
%     \begin{subfigure}[t]{0.45\textwidth}
%     \begin{center}
%     \includegraphics[width=\linewidth]{pathtofigs/selection_camvid.pdf}
%     \end{center}
%     \caption{}
%     \label{fig:selection_camvid_main}
%     \end{subfigure}
%     \begin{subfigure}[t]{0.45\textwidth}
%     \begin{center}
%     \includegraphics[width=\linewidth]{pathtofigs/selection_cityscapes.pdf}
%     \end{center}
%     \caption{}
%     \label{fig:selection_cityscapes_main}
%     \end{subfigure}
%     \caption{Number of class-wise annotations per labeling cycle on (a) CamVid and (b) CityScapes datasets.}
% \end{figure}

==> WACV 2023/fig/selections.tex <==
\begin{figure*}[t]
    \centering
    \begin{subfigure}{0.35\textwidth}
        \begin{center}
        \includegraphics[width=\linewidth]{pathtofigs/selection_camvid.pdf}
        \end{center}
        \caption{CamVid}
        \label{fig:selection_dataset_camvid}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.55\textwidth}
        \begin{center}
        \includegraphics[width=\linewidth]{pathtofigs/selection_cityscapes.pdf}
        \end{center}
        \caption{CityScapes}
        \label{fig:selection_dataset_cityscapes}
    \end{subfigure}
\caption{What does the network want? We visualize the region-wise samples per active learning cycle on both datasets for our main split}
\label{fig:selection_dataset}
\end{figure*}

==> WACV 2023/fig/teaser.tex <==
\begin{figure}[t]
\begin{center}
\includegraphics[width=\linewidth]{pathtofigs/fig_teaser.pdf}
\end{center}
\caption{
Our active learning approach aims to minimize the number of manual region annotations by using pseudo labels for unlabeled data during training phase. Blending (a) the traditional active learning approach with (b) the traditional semi-supervised approach, (c) our approach used semi-supervised learning on the unlabeled data to generate (d) region acquisition scores that can be queued for human annotations.}
\label{fig:teaser_frontpage}
\end{figure}

==> WACV 2023/fig/viz_datasets.tex <==
\begin{figure*}[t]
    \centering
    \begin{subfigure}[t]{0.24\textwidth}
        \begin{center}
        \includegraphics[width=\linewidth]{visuals/camvid/0001TP_008820.png}
        \end{center}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.24\textwidth}
        \begin{center}
        \includegraphics[width=\linewidth]{visuals/camvid/0001TP_008820_gt.png}
        \end{center}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.24\textwidth}
        \begin{center}
        \includegraphics[width=\linewidth]{visuals/camvid/0001TP_008820_sup.png}
        \end{center}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.24\textwidth}
        \begin{center}
        \includegraphics[width=\linewidth]{visuals/camvid/0001TP_008820_semisup.png}
        \end{center}
    \end{subfigure}
    \vspace*{\fill}
    \begin{subfigure}[t]{0.24\textwidth}
        \begin{center}
        \includegraphics[width=\linewidth]{visuals/camvid/0001TP_009780.png}
        \end{center}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.24\textwidth}
        \begin{center}
        \includegraphics[width=\linewidth]{visuals/camvid/0001TP_009780_gt.png}
        \end{center}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.24\textwidth}
        \begin{center}
        \includegraphics[width=\linewidth]{visuals/camvid/0001TP_009780_sup.png}
        \end{center}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.24\textwidth}
        \begin{center}
        \includegraphics[width=\linewidth]{visuals/camvid/0001TP_009780_semisup.png}
        \end{center}
    \end{subfigure}
    \vspace*{\fill}
    \begin{subfigure}[t]{0.24\textwidth}
        \begin{center}
        \includegraphics[width=\linewidth]{visuals/camvid/Seq05VD_f04890.png}
        \end{center}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.24\textwidth}
        \begin{center}
        \includegraphics[width=\linewidth]{visuals/camvid/Seq05VD_f04890_gt.png}
        \end{center}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.24\textwidth}
        \begin{center}
        \includegraphics[width=\linewidth]{visuals/camvid/Seq05VD_f04890_sup.png}
        \end{center}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.24\textwidth}
        \begin{center}
        \includegraphics[width=\linewidth]{visuals/camvid/Seq05VD_f04890_semisup.png}
        \end{center}
    \end{subfigure}
    \vspace*{\fill}
    \begin{subfigure}[t]{0.24\textwidth}
        \begin{center}
        \includegraphics[width=\linewidth]{visuals/camvid/Seq05VD_f03600.png}
        \end{center}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.24\textwidth}
        \begin{center}
        \includegraphics[width=\linewidth]{visuals/camvid/Seq05VD_f03600_gt.png}
        \end{center}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.24\textwidth}
        \begin{center}
        \includegraphics[width=\linewidth]{visuals/camvid/Seq05VD_f03600_sup.png}
        \end{center}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.24\textwidth}
        \begin{center}
        \includegraphics[width=\linewidth]{visuals/camvid/Seq05VD_f03600_semisup.png}
        \end{center}
    \end{subfigure}
\caption{Examples of semantic segmentation outputs on CamVid, the columns represent the image (left), the ground truth (center-left), the predictions of a supervised network (center-right), and the predictions of a network trained via S4AL (right).}
\label{fig:viz_dataset_camvid}
\end{figure*}

\begin{figure*}[t]
    \centering
    \begin{subfigure}[t]{0.24\textwidth}
        \begin{center}
        \includegraphics[width=\linewidth]{visuals/cityscapes/9.png}
        \end{center}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.24\textwidth}
        \begin{center}
        \includegraphics[width=\linewidth]{visuals/cityscapes/9_gt.png}
        \end{center}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.24\textwidth}
        \begin{center}
        \includegraphics[width=\linewidth]{visuals/cityscapes/9_sup.png}
        \end{center}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.24\textwidth}
        \begin{center}
        \includegraphics[width=\linewidth]{visuals/cityscapes/9_semisup.png}
        \end{center}
    \end{subfigure}
    \vspace*{\fill}
    \begin{subfigure}[t]{0.24\textwidth}
        \begin{center}
        \includegraphics[width=\linewidth]{visuals/cityscapes/78.png}
        \end{center}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.24\textwidth}
        \begin{center}
        \includegraphics[width=\linewidth]{visuals/cityscapes/78_gt.png}
        \end{center}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.24\textwidth}
        \begin{center}
        \includegraphics[width=\linewidth]{visuals/cityscapes/78_sup.png}
        \end{center}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.24\textwidth}
        \begin{center}
        \includegraphics[width=\linewidth]{visuals/cityscapes/78_semisup.png}
        \end{center}
    \end{subfigure}
    \vspace*{\fill}
    \begin{subfigure}[t]{0.24\textwidth}
        \begin{center}
        \includegraphics[width=\linewidth]{visuals/cityscapes/389.png}
        \end{center}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.24\textwidth}
        \begin{center}
        \includegraphics[width=\linewidth]{visuals/cityscapes/389_gt.png}
        \end{center}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.24\textwidth}
        \begin{center}
        \includegraphics[width=\linewidth]{visuals/cityscapes/389_sup.png}
        \end{center}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.24\textwidth}
        \begin{center}
        \includegraphics[width=\linewidth]{visuals/cityscapes/389_semisup.png}
        \end{center}
    \end{subfigure}
    \vspace*{\fill}
    \begin{subfigure}[t]{0.24\textwidth}
        \begin{center}
        \includegraphics[width=\linewidth]{visuals/cityscapes/228.png}
        \end{center}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.24\textwidth}
        \begin{center}
        \includegraphics[width=\linewidth]{visuals/cityscapes/228_gt.png}
        \end{center}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.24\textwidth}
        \begin{center}
        \includegraphics[width=\linewidth]{visuals/cityscapes/228_sup.png}
        \end{center}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.24\textwidth}
        \begin{center}
        \includegraphics[width=\linewidth]{visuals/cityscapes/228_semisup.png}
        \end{center}
    \end{subfigure}
\caption{Examples of semantic segmentation outputs on CityScapes, the columns represent the image (left), the ground truth (center-left), the predictions of a supervised network (center-right), and the predictions of a network trained via S4AL (right).}
\label{fig:viz_dataset_cityscapes}
\end{figure*}

==> WACV 2023/tab/additionalresults.tex <==
\begin{table}[t]
    \caption{\textbf{Discussions:} of additional studies conducted on CamVid and CityScapes dataset. We use MobileNetv2 for all our experiments.}
    \begin{subtable}[t]{0.45\textwidth}
        \def\arraystretch{1.2}  
        \small
        \centering
        \caption{\textbf{IoU:} with respect to different block sampling ratios on CamVid and CityScapes datasets.}
        \label{tab:regionsize_camvid_cityscapes}
        \resizebox{\textwidth}{!}{%
        \begin{tabular}{lllll}
        CamVid & mIoU & CityScapes & mIoU \\ \shline
        30 $\times$ 30 $\times$ 2 & 60.4 $\pm$ 1.4 & 43 $\times$ 43 $\times$ 2 & 61.8 $\pm$ 0.8\\
        30 $\times$ 30 $\times$ 4 & 61.4 $\pm$ 0.6 & 43 $\times$ 43 $\times$ 4 & 62.6 $\pm$ 2.2\\
        60 $\times$ 60 $\times$ 1 & 60.8 $\pm$ 2.4 & 86 $\times$ 86 $\times$ 1 & 61.4 $\pm$ 1.6 \\ \bottomrule
        \end{tabular}%
        }
     \end{subtable}
     \\
     \\
     \begin{subtable}[t]{0.3\textwidth}
        \def\arraystretch{1.2}  
        \small
        \centering
        \caption{\textbf{IoU:} with respect to different sampling schemes on CamVid and CityScapes datasets.}
        \label{tab:acquisition_fxs}
        \resizebox{\textwidth}{!}{%
        \begin{tabular}{@{}lll@{}}
         & \multicolumn{2}{c}{mIoU} \\ 
         & CamVid & CityScapes \\ \shline
        Random & 59.1 $\pm$ 1.8 & 59.8 $\pm$ 2.5 \\
        LS & 60.5 $\pm$ 0.5 & 60.3 $\pm$ 1.4  \\
        Ent & 61.2 $\pm$ 0.5 & 62.5 $\pm$ 1.8 \\
        Margin & 60.8 $\pm$ 0.6 & 61.8 $\pm$ 0.5 \\ \bottomrule
        \end{tabular}%
        }
     \end{subtable}
\end{table}

==> WACV 2023/tab/compiled_results.tex <==
\begin{table*}[t]
    \caption{\textbf{Discussions:} of various studies conducted on CamVid and CityScapes dataset. We use MobileNetv2 for all our experiments, except in Table \ref{tab:comparisons_drn_approaches}.}
    \label{tab:compiled_results}
    \begin{subtable}[t]{0.30\textwidth}
        \def\arraystretch{1.2}
        \small
        \caption{\textbf{Region vs Image:} the entire dataset, with top three classes with the largest difference in IoU and (Recall).}
        \label{tab:regionvsimage_camvid}
        \centering
        \resizebox{\textwidth}{!}{%
        \begin{tabular}{@{}lll@{}}
         & \multicolumn{2}{c}{IoU} \\ 
         & Region & Image \\ \shline
        CamVid & 61.78 & 60.31 \\
        $\cdot$ Sign & 40.27 (73.75) & 34.66 (75.22) \\
        $\cdot$ Pedestrian & 49.96 (70.30) & 43.99 (68.29) \\
        $\cdot$ Bicyclist & 51.31 (77.14) & 49.76 (72.08) \\ \bottomrule
        \end{tabular}%
        }
        \end{subtable}
    \hfill
    \begin{subtable}[t]{0.30\textwidth}
        \def\arraystretch{1.2}  
        \small
        \caption{\textbf{Region vs Image:} the entire dataset, with top three classes with the largest difference in IoU and (Recall).}
        \label{tab:regionvsimage_cityscapes}
        \centering
        \resizebox{\textwidth}{!}{%
        \begin{tabular}{@{}lll@{}}
         & \multicolumn{2}{c}{IoU} \\ 
         & Region & Image \\ \shline
        CityScapes & 64.70 & 64.73 \\
        $\cdot$ Truck & 66.07 (85.17) & 60.12 (74.77) \\
        $\cdot$ Bus & 65.31 (89.05) & 67.13 (81.91) \\
        $\cdot$ Train & 46.03 (51.07) & 57.30 (66.67) \\ \bottomrule
        \end{tabular}%
        }
        
     \end{subtable}
     \hfill
     \begin{subtable}[t]{0.36\textwidth}
        \def\arraystretch{1.2}  
        \small
        \caption{\textbf{IoU:} using DRN on VAAL \cite{sinha2019variational} and MAL \cite{ebrahimi2020minimax}. IoU$_s$ indicates the score at starting with 10\% of the data, IoU$_f$ indicates the score at end of active learning, IoU$_{sup}$ are the scores with fully supervised data, and the last row indicates the amount of data utilized.}
        \label{tab:comparisons_drn_approaches}
        \centering
        \resizebox{\textwidth}{!}{%
        \begin{tabular}{@{}llll@{}}
        \\
        \multicolumn{1}{c}{} & VAAL \cite{sinha2019variational} & MAL \cite{ebrahimi2020minimax} & \textbf{S4AL} \\ \shline
        IoU$_s$ & 46.2 & 48.9 & 57.9 \\
        IoU$_f$ & 56.5 {\color[HTML]{32CB00}($+$10.3)} & 58.4 {\color[HTML]{32CB00}($+$9.5)} & 65.7 {\color[HTML]{32CB00}($+$7.8)} \\
        IoU$_{sup}$ & 62.95 $\pm$ 0.70 & 61.9 $\pm$ 0.70 & 67.68 $\pm$ 1.2 \\
        \% data & 40 & 30 & 16 \\ \bottomrule
        \end{tabular}%
        }
        
    \end{subtable}

\end{table*}

==> WACV 2023/tab/sota_cityscapes.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
%\def\arraystretch{1.2}

% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table*}[t]
\tiny
\caption{\textbf{IoU:} Class-wise and mean on CityScapes using MobileNetv2 - while all approaches use 40\% data to achiever their goal, we achieve our goal with only 16\% data.}
\label{tab:results_cityscapes}
\def\arraystretch{1.2}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lcccccccccc}
Method & Road & \begin{tabular}[c]{@{}c@{}}Side\\ walk\end{tabular} & Building & Wall & Fence & Pole & \begin{tabular}[c]{@{}c@{}}Traffic\\ Light\end{tabular} & \begin{tabular}[c]{@{}c@{}}Traffic\\ Sign\end{tabular} & Vegetation & Terrain \\ \shline
{\color[HTML]{9B9B9B} Supervised} & {\color[HTML]{9B9B9B} 97.58} & {\color[HTML]{9B9B9B} 80.55} & {\color[HTML]{9B9B9B} 88.43} & {\color[HTML]{9B9B9B} 51.22} & {\color[HTML]{9B9B9B} 47.61} & {\color[HTML]{9B9B9B} 35.19} & {\color[HTML]{9B9B9B} 42.19} & {\color[HTML]{9B9B9B} 56.79} & {\color[HTML]{9B9B9B} 89.41} & {\color[HTML]{9B9B9B} 60.22} \\
Random & 96.03 & 72.36 & 86.79 & 43.56 & 44.22 & 36.99 & 35.28 & 53.87 & 86.91 & 54.58 \\
Entropy & 96.28 & 73.31 & 87.13 & 43.82 & 43.87 & 38.10 & 37.74 & 55.39 & 87.52 & 53.68 \\
Core-Set \cite{sener2018active} & 96.12 & 72.76 & 87.03 & 44.86 & 45.86 & 35.84 & 34.81 & 53.07 & 87.18 & 53.49 \\
% VAAL \cite{sinha2019variational} & 96.22 & 73.27 & 86.95 & 47.27 & 43.92 & 37.40 & 36.88 & 54.90 & 87.10 & 54.48 \\
DEAL \cite{xie2020deal} & 95.89 & 71.69 & 87.09 & 45.61 & 44.94 & 38.29 & 36.51 & 55.47 & 87.53 & 56.90 \\
\textbf{S4AL} & 97.73 & 81.76 & 88.63 & 51.42 & 47.40 & 36.00 & 43.91 & 58.27 & 89.72 & 62.01 \\ \hline
% \end{tabular}%
% }
% \label{tab:results_cityscapes_1}
% \end{table*}

% % Please add the following required packages to your document preamble:
% % \usepackage{graphicx}
% \begin{table*}[t]
% \tiny
% \def\arraystretch{1.2}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{lcccccccccc}

 & Sky & \begin{tabular}[c]{@{}c@{}}Pedes-\\ trian\end{tabular} & Rider & Car & Truck & Bus & Train & \begin{tabular}[c]{@{}c@{}}Motor-\\ Cycle\end{tabular} & Bicycle & mIoU \\ \shline
{\color[HTML]{9B9B9B} Supervised} & {\color[HTML]{9B9B9B} 92.69} & {\color[HTML]{9B9B9B} 65.12} & {\color[HTML]{9B9B9B} 37.32} & {\color[HTML]{9B9B9B} 90.67} & {\color[HTML]{9B9B9B} 66.24} & {\color[HTML]{9B9B9B} 71.84} & {\color[HTML]{9B9B9B} 63.84} & {\color[HTML]{9B9B9B} 42.35} & {\color[HTML]{9B9B9B} 61.84} & {\color[HTML]{9B9B9B} 65.30} \\

Random & 91.47 & 62.74 & 37.51 & 88.05 & 56.64 & 61.00 & 43.69 & 30.58 & 55.67 & 59.00 \\
Entropy & 92.05 & 63.96 & 34.44 & 88.38 & 59.38 & 64.64 & 50.80 & 36.13 & 57.10 & 61.46 \\
Core-Set \cite{sener2018active} & 91.89 & 62.48 & 36.28 & 87.63 & 57.25 & 67.02 & 56.59 & 29.34 & 53.56 & 60.69 \\
% VAAL \cite{sinha2019variational} & 91.63 & 63.44 & 38.92 & 87.92 & 50.15 & 63.70 & 52.36 & 35.99 & 54.97 & 60.92 \\
DEAL \cite{xie2020deal} & 91.78 & 64.25 & 39.77 & 88.11 & 56.87 & 64.46 & 50.39 & 38.92 & 56.59 & 61.64 \\
\textbf{S4AL} & 92.81 & 65.62 & 39.71 & 90.52 & 66.07 & 65.31 & 46.03 & 46.88 & 61.77 & 64.80 \\ \hline
\end{tabular}%
}
\end{table*}

==> WACV 2023/tab/training_settings.tex <==
\begin{table}
\small
\caption{Supervised Learning parameters.}
\label{tab:supervised_settings}
\def\arraystretch{1.2}
\centering
\resizebox{0.45\textwidth}{!}{%
\begin{tabular}{@{}lll@{}}
Config & CamVid & CityScapes \\ \shline
Learing Rate & $1e-2$ & $1e-2$ \\
Optimizer & SGD & SGD \\
Scheduler & PolyLR & PolyLR \\
 &  &  \\
Batch Size & 4 & 4 \\
Epoch Iterations & 100 & 200 \\
Epochs & 100 & 100 \\
 &  &  \\
Augmentations & \begin{tabular}[c]{@{}l@{}}Resize({[}0.75,1.25{]}),\\ ColorJitter(p = 0.5),\\ HFlip(p = 0.5)\end{tabular} & \begin{tabular}[c]{@{}l@{}}Resize({[}0.5,2.0{]}),\\ ColorJitter(p = 0.5),\\ HFlip(p = 0.5)\end{tabular} \\ \bottomrule
\end{tabular}%
}
\end{table}

\begin{table}[t]
\small
\caption{Active Learning with Semi-Supervised Learning parameters.}
\label{tab:semisup_al_settings}
\def\arraystretch{1.2}
\centering
\resizebox{0.45\textwidth}{!}{%
\begin{tabular}{@{}lll@{}}
Config & CamVid & CityScapes \\ \shline
Learing Rate & 1e-2 & 1e-2 \\
Optimizer & SGD & SGD \\
Scheduler & PolyLR & PolyLR \\
 &  &  \\
Batch Size (Labeled) & 4 & 4 \\
Batch Size (Un-Labeled) & 4 & 4 \\
Epoch Iterations & 50 & 100 \\
Epochs & 100 & 100 \\
Coldstart Epochs & 10 & 10 \\
Final Cycle Epochs & 200 & 200 \\
 &  &  \\
Active Learning Cycles & 2 & 5 \\
Active Learning Regions & 30 $\times$ 30 $\times$ 4 & 43 $\times$ 43 $\times$ 4 \\
 &  &  \\
\begin{tabular}[c]{@{}l@{}}Augmentations\\ (Labeled)\end{tabular} & \begin{tabular}[c]{@{}l@{}}Resize({[}0.75,1.25{]}),\\ ColorJitter(p = 0.5),\\ HFlip(p = 0.5)\end{tabular} & \begin{tabular}[c]{@{}l@{}}Resize({[}0.5,2.0{]}),\\ ColorJitter(p = 0.5),\\ HFlip(p = 0.5)\end{tabular} \\
 &  &  \\
\begin{tabular}[c]{@{}l@{}}Weak Augmentations\\ (Un-Labeled)\end{tabular} & \begin{tabular}[c]{@{}l@{}}Resize({[}0.75,1.25{]}),\\ HFlip(p = 0.5)\end{tabular} & \begin{tabular}[c]{@{}l@{}}Resize({[}0.5,2.0{]}),\\ HFlip(p = 0.5)\end{tabular} \\
 &  &  \\
\begin{tabular}[c]{@{}l@{}}Strong Augmentations\\ (Un-Labeled)\end{tabular} & \begin{tabular}[c]{@{}l@{}}Resize({[}0.75,1.25{]}),\\ ColorJitter(p = 0.5),\\ HFlip(p = 0.5),\\ ClassMix\cite{Olsson_2021_WACV}\end{tabular} & \begin{tabular}[c]{@{}l@{}}Resize({[}0.5,2.0{]}),\\ ColorJitter(p = 0.5),\\ HFlip(p = 0.5),\\ ClassMix\cite{Olsson_2021_WACV}\end{tabular} \\
 &  &  \\
Replay Buffer Size & 50 & 500 \\ \bottomrule
\end{tabular}%
}

\end{table}

==> fig/cityscapes_selections.tex <==
\begin{figure}[t]
    \centering
    \begin{subfigure}[t]{0.23\linewidth}
        \begin{center}
        \includegraphics[width=\linewidth]{pathtofigs/cityscapes_selections/69.png}
        \end{center}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.23\linewidth}
        \begin{center}
        \includegraphics[width=\linewidth]{pathtofigs/cityscapes_selections/112.png}
        \end{center}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.23\linewidth}
        \begin{center}
        \includegraphics[width=\linewidth]{pathtofigs/cityscapes_selections/1862.png}
        \end{center}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.23\linewidth}
        \begin{center}
        \includegraphics[width=\linewidth]{pathtofigs/cityscapes_selections/2072.png}
        \end{center}
    \end{subfigure}
    \par\medskip
    \begin{subfigure}[t]{0.23\linewidth}
        \begin{center}
        \includegraphics[width=\linewidth]{pathtofigs/cityscapes_selections/69_mask.png}
        \end{center}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.23\linewidth}
        \begin{center}
        \includegraphics[width=\linewidth]{pathtofigs/cityscapes_selections/112_mask.png}
        \end{center}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.23\linewidth}
        \begin{center}
        \includegraphics[width=\linewidth]{pathtofigs/cityscapes_selections/1862_mask.png}
        \end{center}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.23\linewidth}
        \begin{center}
        \includegraphics[width=\linewidth]{pathtofigs/cityscapes_selections/2072_mask.png}
        \end{center}
    \end{subfigure}
    \par\medskip
    \begin{subfigure}[t]{0.23\linewidth}
        \begin{center}
        \includegraphics[width=\linewidth]{pathtofigs/cityscapes_selections/69_drn.png}
        \end{center}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.23\linewidth}
        \begin{center}
        \includegraphics[width=\linewidth]{pathtofigs/cityscapes_selections/112_drn.png}
        \end{center}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.23\linewidth}
        \begin{center}
        \includegraphics[width=\linewidth]{pathtofigs/cityscapes_selections/1862_drn.png}
        \end{center}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.23\linewidth}
        \begin{center}
        \includegraphics[width=\linewidth]{pathtofigs/cityscapes_selections/2072_drn.png}
        \end{center}
    \end{subfigure}
\caption{\textbf{Regions:} Set of images showing what areas were chosen to be sampled in CityScapes over 5 active learning cycles with MobileNetv2 (2nd row) and DRN (3rd row). Our approach focuses on regions with high value information, still having uniqueness with areas acquisitioned depending on the backbone being used.}
\label{fig:selection_cityscapes_regions}
\end{figure}
